Dual Distribution Alignment Network for Generalizable Person Re-Identification

Domain generalization (DG) serves as a promising solution to handle person Re-Identification (Re-ID), which trains the model using labels from the source domain alone, and then directly adopts the trained model to the target domain without model updating. However, existing DG approaches are usually disturbed by serious domain variations due to significant dataset variations. Subsequently, DG highly relies on designing domain-invariant features, which is however not well exploited, since most existing approaches directly mix multiple datasets to train DG based models without considering the local dataset similarities, i.e., examples that are very similar but from different domains. In this paper, we present a Dual Distribution Alignment Network (DDAN), which handles this challenge by mapping images into a domain-invariant feature space by selectively aligning distributions of multiple source domains. Such an alignment is conducted by dual-level constraints, i.e., the domain-wise adversarial feature learning and the identity-wise similarity enhancement. We evaluate our DDAN on a large-scale Domain Generalization Re-ID (DG Re-ID) benchmark. Quantitative results demonstrate that the proposed DDAN can well align the distributions of various source domains, and significantly outperforms all existing domain generalization approaches.

==> 3_related_new.tex <==
\section{Related Work}
\noindent{\textbf{Person Re-identification.}}
Along with the success of deep CNNs~\cite{conf/cvpr/Bak017,conf/cvpr/BaiBT17,conf/ijcai/LiZG17}, person Re-ID has achieved remarkable performance under the \emph{i.i.d.}~assumption between training and test data. However, the learned models commonly overfit to the training dataset, and might perform poorly when directly applied to unseen datasets.
%
Therefore, UDA approaches are proposed for person Re-ID ~\cite{conf/bmvc/LinLLK18,conf/cvpr/WangZGL18,conf/eccv/BakCL18}. 
% 下面这句话改成： A UDA model involves a labeled source domain and an unlabeled target domain, 但它任需要收集target的数据集，且当target数据集过小时，效果不好。因此，【song】提出了DG的方法。可以不需要任何target域上的信息，而将模型直接运用在unseen domain
In such a setting, a labeled source domain is involved to help the model to fit the distribution of an unlabeled target domain. However, UDA approaches typically require a large amount of target data to achieve satisfactory results by avoiding overfitting to the source data.
%
% To this end, \cite{conf/cvpr/SongYSXH19} introduced a DG model to person Re-ID, which is trained using multiple source domain datasets and is expected to perform well in the unseen target domain without any updating, \emph{i.e.}, adaptation or retraining.
% To this end, the more realistic DG setting was introduced  to person Re-ID.
% A UDA model involves a labeled source domain and an unlabeled target domain. However, 

% -----思路-------
% 1. 先大概提一下DG是什么
% 2. 现在的DG大都在分类里面 (说我们的domain和他们不一样的地方)
% 3. 最近才刚开始出现reid的DG 
% 4. 我们的东西与上述的不一样的地方
\noindent{\textbf{Domain Generalization.}}
% 1. 先大概提一下DG是什么
DG methods aim to learn a generalizable model, which should remove the domain-shift among different domains without needing the data of target domain during the training phase. 
% (上面一句话好像没什么毛病，然后补一句:)已经有很多 不同的 针对分类问题的DG的方法被提出来：
% 2. 现在的DG大都在分类里面 (说我们的domain和他们不一样的地方)
In this regard, many methods have been proposed to conduct DG for the classification task,
%
%\red{\cite{conf/eccv/XuLNX14} trained a model for each source domain and select the best one for each target domain during the test phase.} 
%检查：下面是说分类的
% More efficient choices exist as well, such as learning a model to extract task-specific and domain-invariant features:
% \cite{conf/icml/MuandetBS13} proposed to learn features via kennel-based optimization; \cite{conf/iccv/GhifaryKZB15} learned a multi-task auto-encoder to extract domain-invariant features; \cite{conf/ijcai/YangG13} proposed to use canonical correlation analysis (CCA) as a domain-distance regularization for DG.
%More efficient choices exist as well, 
such as kernel-based optimization~\cite{conf/icml/MuandetBS13}, canonical correlation analysis~\cite{conf/ijcai/YangG13} and multi-task auto-encoder~\cite{conf/iccv/GhifaryKZB15}.
Besides, model-agnostic meta-learning~\cite{conf/icml/FinnAL17} was also introduced~\cite{conf/icml/LiYZH19,journals/corr/abs-1910-13580}.
%
% 下面这两篇是pair-wise拉近的两篇
% Adversarial learning也是一种常见的方法：
As another innovation, the adversarial feature alignment~\cite{conf/cvpr/LiPWK18,conf/eccv/LiTGLLZT18} trains a domain-invariant model by reducing the pairwise domain discrepancy with either MMD or JSD.
% 修改：这里是trade-off的那篇: [引用]指出，在domain-invariance和classification accuracy中存在trade-off, 如果一味地考虑domain-invariacne会导致精度下降，所以他们介绍了...
In response to the popularization of domain-invariance based approaches, \cite{journals/corr/abs-1904-12543} revealed that there is a statistical trade-off between domain-invariance and classification accuracy.
% 补充：（这里引入我们的东西合适吗？）这样的问题同样在reid中出现，我们发现如果以pair-wise的形式来对齐分布，会因为分布变化过大而导致feature的可判别力下降，因此在我们的方法中，我们提出了一个xx(这个词早上是不是有提过？)的domain-wise distribution alignment. 选择一个central domain, 使得对齐分布过程中尽量减少分布的变化，在对齐分布的同时能够保证特征的可判别力（或者说有效性？）。
We have observed the same problem in person Re-ID: The pairwise domain alignment can reduce the feature discriminability, as it needs extensive distributional shifts to align different Re-ID datasets.

%
%下面说reid:
% 补充：最近，DG方面的reid也开始引起关注：
% Note that the existing methods are designed for the classification task. In contrast, DG problem in person Re-ID should handle the retrieval task, which has fundamental difference.
% 修改+补充：[song 引用]的文章，使用了meta-learning，同时 "DIMN generates classifier weights from gallery images and then takes the dot product of the classifier weights and probe image features to calculate matching scores"， 但使用meta-learning pipeline 来保证domain-invariant使得优化变得复杂，且在测试时速度很慢。因此， ~\cite{journals/corr/abs-1905-03422} 提出了一种简单的方法，直接在网络里加入IN和BN， 来改善提高performance。
To handle person Re-ID, DIMN~\cite{conf/cvpr/SongYSXH19} adopted meta-learning to learn the classifier from the gallery images, which outputs matching scores by the dot product between features of the gallery and the probe images. However, such a scheme can increase the complexity of optimization, and greatly lower the test speed correspondingly. 
%
As a more straightforward alternative, DualNorm~\cite{journals/corr/abs-1905-03422} employed both the instance and batch normalization layers %(IN)~\cite{journals/corr/UlyanovVL16} 
% and Batch Normalization (BN)~\cite{conf/icml/IoffeS15} 
to improve the DG performance of the feature extractor.

% 补充：与他们的方法不同，我们考虑以dual domain distribution alignment的方法来消除domain shift并获取domain-invariant feature. 由于reid与分类的差异性(或者直接说由于reid数据集的特殊性？), 我们不仅设计了一个xxx的domain-wise distribution alignment, 同时，还考虑到了局部identity的相似性..(这样够了么？)
Our DDAN is distinguished to the above methods in two folds: At the domain level, instead of adopting the pairwise alignment, we selectively reduce the discrepancy between a \emph{central} domain and the \emph{peripheral} domains, such that the loss of distinguishability is minimized. At the identity level, differing from existing methods that directly mix all source datasets, we also consider the local similarities between identities in different domains, which is quantitatively proven to be very effective in promoting the feature discriminability.
